An Agentic AI Scientific Community for Automated Neural Operator Discovery

We present an agentic approach to autonomous neural operator discovery based on an AI scientific community, which consists of a swarm of virtual laboratories that interact under a citation-based economy of influence. Highly-cited labs found new labs that follow their research direction and replace non-performing labs. Each virtual lab contains three agents: an LLM planner that proposes an architecture, a numerical worker that trains and measures it, and an LLM reviewer that participates in cross-lab peer review. All labs share a common vocabulary consisting of DeepONet (branch-trunk), Fourier, Transformer (attention), wavelet, and residual convolutional neural operator building blocks. We evaluate the neural operator AI scientific community on five problems, namely piecewise regression, the linear advection and Burgers 1D PDEs, and the Navier-Stokes and Darcy flow 2D PDEs, while repeating the simulation three times for each problem. The results show that the neural operator AI scientific community is capable of discovering high-accuracy, low-parameter-count neural operator architectures. All 9,623 LLM calls are logged and audited, which reveals that the virtual lab LLM planners choose to hybridize in 99.8% of their logged decisions, consistently returning multi-family hybrids. Moreover, we conducted an ablation study by replacing the LLM agents in each lab by rule-based alternatives, which caused the scientific community to collapse to non-hybridized single-family stacks in several cases, showing that LLM agency is needed to preserve diversity. The results suggest a no-free-lunch theorem for neural operators: there is no universal winner. The code, configurations, and the complete LLM transcripts are released at https://github.com/luislootx/AI-SC.

==> tab_actions.tex <==
\begin{tabular}{lcc}
\toprule
Problem & \textsc{explore} & \textsc{hybridize} \\
\midrule
Piecewise Reg. (1D) & 0\% & 100\% \\
Advection (1D) & 0\% & 100\% \\
Burgers (1D) & 0\% & 100\% \\
Navier-Stokes (2D) & 0\% & 100\% \\
Darcy (2D) & 0\% & 100\% \\
\midrule
\textbf{all} & 0\% & 100\% \\
\bottomrule
\end{tabular}

==> tab_baselines.tex <==
\begin{tabular}{lrcc}
\toprule
Model & Params & NS-2D rel.\ $L_2$ & Darcy-2D rel.\ $L_2$ \\
\midrule
Discovered hybrid (Darcy) & 1.3M & 0.0018$\pm$0.0002 & 0.0631$\pm$0.0083 \\
Discovered hybrid (NS) & 1.1M & 0.0005$\pm$0.0000 & 0.7127$\pm$0.0736 \\
DeepONet & 603K & 0.1613$\pm$0.0122 & 0.0649$\pm$0.0037 \\
POD-DeepONet & 142K & 0.0033$\pm$0.0001 & 0.0819$\pm$0.0028 \\
FNO & 1.2M & 0.0002$\pm$0.0000 & 0.3070$\pm$0.0404 \\
Transformer & 105K & 0.2624$\pm$0.0038 & 0.5207$\pm$0.0102 \\
\bottomrule
\end{tabular}

==> tab_discovery.tex <==
\begin{tabular}{lcccc}
\toprule
Problem & \multicolumn{2}{c}{Relative $L_2$ error} & \multicolumn{2}{c}{Parameter count} \\\cline{2-5}\\[-2ex]
 & LLM & rule-based & LLM & rule-based \\
\midrule
Piecewise Reg. (1D) & 0.0417$\pm$0.0011 & 0.0405$\pm$0.0007 & 487K$\pm$258K & 198K$\pm$95K \\
Advection (1D) & 0.0159$\pm$0.0038 & 0.0183$\pm$0.0007 & 273K$\pm$157K & 456K$\pm$159K \\
Burgers (1D) & 0.0799$\pm$0.0067 & 0.0709$\pm$0.0047 & 472K$\pm$415K & 197K$\pm$103K \\
Navier-Stokes (2D) & 0.0009$\pm$0.0005 & 0.0007$\pm$0.0000 & 2.2M$\pm$613K & 5.6M$\pm$4.1M \\
Darcy (2D) & 0.0095$\pm$0.0003 & 0.0096$\pm$0.0015 & 1.4M$\pm$403K & 966K$\pm$593K \\
\bottomrule
\end{tabular}

==> tab_evidence.tex <==
\begin{tabular}{lcccc}
\toprule
LLM run & planner & reviewer & parse-ok & fallbacks \\
\midrule
\texttt{advec seed137} & 320 & 320 & 640/640 & 0 \\
\texttt{advec seed2024} & 320 & 320 & 640/640 & 0 \\
\texttt{advec seed42} & 320 & 320 & 640/640 & 0 \\
\texttt{burgers seed137} & 320 & 320 & 640/640 & 0 \\
\texttt{burgers seed2024} & 320 & 320 & 640/640 & 0 \\
\texttt{burgers seed42} & 320 & 320 & 640/640 & 0 \\
\texttt{darcy seed137} & 335 & 326 & 661/661 & 0 \\
\texttt{darcy seed2024} & 320 & 320 & 640/640 & 0 \\
\texttt{darcy seed42} & 320 & 320 & 640/640 & 0 \\
\texttt{ns seed137} & 320 & 320 & 640/640 & 0 \\
\texttt{ns seed2024} & 320 & 320 & 640/640 & 0 \\
\texttt{ns seed42} & 320 & 320 & 640/640 & 0 \\
\texttt{pwreg seed137} & 320 & 320 & 640/640 & 0 \\
\texttt{pwreg seed2024} & 322 & 320 & 642/642 & 0 \\
\texttt{pwreg seed42} & 320 & 320 & 640/640 & 0 \\
\midrule
\textbf{total} & \multicolumn{3}{c}{9623 LLM calls} & \textbf{0} \\
\bottomrule
\end{tabular}

==> tab_perseed.tex <==
\begin{tabular}{llllcc}
\toprule
Problem & Agents & Seed & Discovered blocks & Rel.\ $L_2$ error & Params \\
\midrule
Piecewise Reg. (1D) & LLM & 42 & \texttt{A-W-R-F} & 0.0429 & 692K \\
Piecewise Reg. (1D) & LLM & 137 & \texttt{R-R-W-T-A} & 0.0419 & 122K \\
Piecewise Reg. (1D) & LLM & 2024 & \texttt{A-R-W-T} & 0.0404 & 647K \\
Piecewise Reg. (1D) & rule-based & 42 & \texttt{W-A-W-W} & 0.0410 & 333K \\
Piecewise Reg. (1D) & rule-based & 137 & \texttt{W-R-W-W-W} & 0.0396 & 128K \\
Piecewise Reg. (1D) & rule-based & 2024 & \texttt{R-W-W-R-W} & 0.0410 & 134K \\
\midrule
Advection (1D) & LLM & 42 & \texttt{F-A-W-T} & 0.0191 & 143K \\
Advection (1D) & LLM & 137 & \texttt{A-R-F-F-T} & 0.0105 & 494K \\
Advection (1D) & LLM & 2024 & \texttt{F-A-W-T} & 0.0180 & 182K \\
Advection (1D) & rule-based & 42 & \texttt{F-A-T-T-T-T} & 0.0186 & 559K \\
Advection (1D) & rule-based & 137 & \texttt{A-F-W-F} & 0.0173 & 576K \\
Advection (1D) & rule-based & 2024 & \texttt{R-F-F} & 0.0189 & 231K \\
\midrule
Burgers (1D) & LLM & 42 & \texttt{F-W-T-F-R-A} & 0.0759 & 1.1M \\
Burgers (1D) & LLM & 137 & \texttt{F-W-A-R} & 0.0745 & 142K \\
Burgers (1D) & LLM & 2024 & \texttt{F-A-T-W} & 0.0894 & 217K \\
Burgers (1D) & rule-based & 42 & \texttt{F-R-F-T-A-F} & 0.0767 & 335K \\
Burgers (1D) & rule-based & 137 & \texttt{F-F-F-T-A} & 0.0707 & 87K \\
Burgers (1D) & rule-based & 2024 & \texttt{F-R-F} & 0.0653 & 169K \\
\midrule
Navier-Stokes (2D) & LLM & 42 & \texttt{F-A-T-W-F} & 0.0011 & 1.4M \\
Navier-Stokes (2D) & LLM & 137 & \texttt{F-A-W-T-R-F} & 0.0003 & 2.6M \\
Navier-Stokes (2D) & LLM & 2024 & \texttt{A-W-T-A-F} & 0.0015 & 2.8M \\
Navier-Stokes (2D) & rule-based & 42 & \texttt{F-F-F-F} & 0.0007 & 10.9M \\
Navier-Stokes (2D) & rule-based & 137 & \texttt{F-W-T-F-F} & 0.0006 & 921K \\
Navier-Stokes (2D) & rule-based & 2024 & \texttt{F-F-F-F} & 0.0007 & 5.1M \\
\midrule
Darcy (2D) & LLM & 42 & \texttt{R-A-W-F} & 0.0099 & 1.9M \\
Darcy (2D) & LLM & 137 & \texttt{A-W-R-F-W} & 0.0091 & 1.3M \\
Darcy (2D) & LLM & 2024 & \texttt{A-W-R-T-F} & 0.0095 & 930K \\
Darcy (2D) & rule-based & 42 & \texttt{W-W-R-R-F} & 0.0089 & 1.7M \\
Darcy (2D) & rule-based & 137 & \texttt{W-W-F-W} & 0.0082 & 933K \\
Darcy (2D) & rule-based & 2024 & \texttt{W-W-W-W} & 0.0116 & 257K \\
\bottomrule
\end{tabular}

==> tab_timing.tex <==
\begin{tabular}{lcccc}
\toprule
Problem & \multicolumn{2}{c}{Total run (min)} & \multicolumn{2}{c}{Per-lab evaluation (sec)} \\\cline{2-5}\\[-2ex]
 & LLM & rule-based & LLM & rule-based \\
\midrule
Piecewise Reg. (1D) & 89.7$\pm$18.3 & 26.0$\pm$11.7 & 19.4$\pm$1.8 & 4.9$\pm$2.4 \\
Advection (1D) & 96.7$\pm$10.6 & 29.2$\pm$12.2 & 18.2$\pm$2.2 & 5.5$\pm$2.4 \\
Burgers (1D) & 108.3$\pm$2.3 & 41.1$\pm$0.9 & 19.8$\pm$1.8 & 7.0$\pm$0.5 \\
Navier-Stokes (2D) & 270.9$\pm$104.3 & 103.1$\pm$6.7 & 51.3$\pm$27.1 & 18.7$\pm$3.3 \\
Darcy (2D) & 173.6$\pm$71.9 & 99.9$\pm$7.9 & 42.1$\pm$15.9 & 18.4$\pm$2.6 \\
\bottomrule
\end{tabular}

==> tab_trainop.tex <==
\begin{tabular}{lc}
\toprule
Operator (NS-2D, screening fidelity) & Train time (s) \\
\midrule
POD-DeepONet & 4.1$\pm$0.0 \\
FNO & 9.7$\pm$0.4 \\
Discovered hybrid (NS) & 20.3$\pm$0.5 \\
Discovered hybrid (Darcy) & 22.5$\pm$0.2 \\
Pure Transformer & 37.4$\pm$0.1 \\
DeepONet & 48.4$\pm$0.7 \\
\bottomrule
\end{tabular}
